Multi-Protocol Location Forwarding (MPLF) for Space Routing

The structure and routing architecture design is critical for achieving low latency and high capacity in future LEO space networks (SNs). Existing studies mainly focus on topologies of space networks, but there is a lack of analysis on constellation structures, which can greatly affect network performance. In addition, some routing architectures are designed for networks with a small number of network nodes such as Iridium while they introduce significant network overhead for high-density networks (i.e., mega-constellation networks containing thousands of satellites). In this paper, we conduct the quantitatively study on the design of network structure and routing architecture in space. The high density, high dynamics, and large scale nature of emerging Space Networks (SNs) pose significant challenges, such as unstable routing paths, low network reachability, high latency, and large jitter. To alleviate the above challenges, we design the structure of space network to maximum the connectivity through wisely adjusting the inter-plane inter satellite link. We further propose Multi-Protocol Location Forwarding (MPLF), a distributed routing architecture, targeting at minimizing the propagation latency with a distributed, convergence-free routing paradigm, while keeping routing stable and maximum the path diversity. Comprehensive experiments are conducted on a customized platform \textit{Space Networking Kits} (SNK) which demonstrate that our solution can outperform existing related schemes by about 14\% reduction of propagation latency and 66\% reduction of hops-count on average, while sustaining a high path diversity with only $O(1)$ time complexity.

==> data/related.tex <==

\section{Background and Related Works}
\label{sec:background}











\subsection{Constellation and Networking Structure Design}


With the advent of multi-satellite systems, i.e., constellations, the traditional orbit design principles focused on a single satellite need to be extended to consider the performance of the entire constellation.
Some constellations \cite{iridium,starlink2,kuiper,telesat} have implemented inter-satellite link (ISL)  for inter-satellite information transfer, at which point the system can be abstracted as a network system, in which the design of space network structure must take into account the motion and traffic characteristics between satellite nodes in the system.

Satellite link establishment does not necessarily follow the principle of closest proximity, and some researchers have studied the constellation topology design, also called Link Assignment, which abstracts the FSA with a finite state machine and uses an optimization method to dynamically adjust the link establishment between satellites according to the load situation \cite{chang1995topological, chang1998fsa}, and the link can be established by satellites within any satellite visual range (LoS).
Bhattacherjee \cite{bhattacherjee2019network} ignored the nearest neighbor principle and proposed a topology design method for the giant constellation network and abstracted it as an integer linear programming problem, using moduli units to reduce the problem complexity for optimization. They also introduce several connectivity metrics for network evaluation.
Although not using the nearest neighbor principle can effectively increase the network throughput and reduce the average hop count of flows, etc., it is more like an extension of the study that mimics the network topology design in highly controllable DCNs \cite{al2008scalable,singla2012jellyfish} and lacks practicality, especially in highly uncontrollable environments in space where it is difficult to apply practically. because it would present additional technical hurdles that are difficult to overcome.
For example, the network overhead of link dynamic adjustment, which can be extremely burdensome when the constellation size rises, and is therefore only suitable for use in constellations with a small number of satellites and interstellar information transmission such as GNSS systems \cite{yan2020integer}.



Although some constellations have planned to implement satellite Internet without using ISL \cite{oneweb}, to achieve relay transmission in the form of Bent-pipe and ground stations, but it is difficult to achieve the performance of ISL system in terms of time delay, throughput, and robustness \cite{bhattacherjee2021towards}.
Therefore, establishing persistent links between neighboring satellites within and between orbits, respectively, is a more practical approach.
The persistent links need to consider the link construction pattern, which generally allows each satellite to establish persistent links with four or six adjacent satellites in a nearest neighbor manner, forming a local topology of Manhattan (+Grid) or triangular Manhattan pattern (*Gird)\cite{wood2001internetworking}. 
However, few works focus on the network structure affected by the configuration of constellation, specifically each satellite is connected to the neighboring satellites, but without considering which phase is connected.
The topology of space networks built on the Manhattan or triangular Manhattan pattern is relatively simple, but in the Walker configuration constellation there is a 'seam' phenomenon, which leads the 'last hop' ambiguity of some geographic information routing algorithms appear dead-end problem \cite{henderson2000distributed,tsunoda2006geographical}.

The structure of space network constructed based on the Manhattan or triangular Manhattan pattern is relatively simple, but there are "seams" in the Walker constellation, leading to dead-end problems in the "last-hop" ambiguity of some geographical routing algorithms \cite{henderson2000distributed,tsunoda2006geographical}, which we will discuss in Section \ref{sec:last_gap}.




\subsection{Routing in Space Networks}

With the popularity of satellite communications, it has become increasingly difficult to work as a simple repeater to meet the diverse requirements of complex communication systems, so space routing has been proposed accordingly.
Early satellite network services, such as the Iridium system, started with connection-oriented services, i.e., packets between arbitrary source and destination nodes would be forwarded along the same path. Some researchers have explored the application of such protocols to space networks, mainly including ATM\cite{mauger1997qos,werner1997dynamic} and MPLS\cite{donner2004mpls}. However, the connection-oriented routing approach is only applicable to smaller networks, and providing centralized computation for networks with many nodes would have a large routing overhead and is therefore not applicable to large-scale constellations.

If connectionless packet forwarding protocols such as IP are applied to space networks, mobility management is the key issue, especially i.e., routing dead ends or last hop problems handled by edge nodes \cite{tsunoda2004supporting,tsunoda2006geographical}.
Traditional IP mobility management policies \cite{rfc3344} require sending application messages when switching new access points, and high dynamics in space networks can cause great network overhead by frequently allowing edge nodes to send application messages.
\cite{tsunoda2004supporting} proposes to establish a mapping of terminal logical IPs to geographic locations, and to make the granularity of the switched cells larger, i.e., from terminals to cells (cells), as a way to reduce the network overhead caused by the large number of binding updates due to the movement of satellite coverage areas. In this way, the original binding update is determined by the switching to the geographical location of the terminal, so it is called Handover-Independent IP Mobility Management. However, since this method does not deal with the last hop thoroughly, based on this \cite{tsunoda2006geographical} introduces a combination of orbit and geographic information, restricting the routing satellite that is close to the destination terminal to the same orbit of the satellite accessed by the destination node, i.e., to ensure the existence of an interplanetary link, to solve this problem. However, this method raises the last-hop problem to the network layer to avoid getting into a dead end by routing methods, which increases the complexity of the routing process.
\cite{yang2016seamless} also proposes an edge mobility management based on SDN architecture, but mainly focuses on seamless switching, in the assumption of getting a global view with GEO, and does not discuss in detail the network address and how addressing is handled.


In network core routing, the connectionless routing algorithms in terrestrial networks have various characteristics \cite{besta2020high}, for example, they can be divided into centralized routing strategies (e.g., link-state routing LS) and decentralized routing strategies (e.g., distance vector routing DV) according to the computational entity.
Under some space routing schemes that consider only the network core, the centralized routing can be applied in some constellation systems with a small number of nodes by using the virtual topology \cite{chang1998fsa,jia2018routing,zhang2020application} of the time slot discrete as a relatively static topology, but if the edge nodes are considered , its dynamics to the space network is difficult to meet. In addition, the large number of nodes under the giant constellation will make this method sharply increase the network overhead, so it is not applicable.

The virtual node method \cite{mauger1997qos} is a strategy for linking terrestrial geographic information to network addressing.
To cope with the non-adaptability of centralized computational routing in satellite networks, Ekici\cite{ekici2000datagram,ekici2001distributed} has designed a distributed, connectionless routing algorithm with an Iridium-like constellation as the topology that can provide the smallest propagation delay path. Its algorithm abstracts the constellation topology as a two-dimensional mesh network, discretizes geographic addresses into logical addresses assigned to each satellite, and generates optimal forwarding paths hop-by-hop based on the relative distance from each node to its destination. This method is a static addressing strategy, which only considers the routing between satellites as forwarding nodes and does not contact the network edge, which is mostly deployed on the ground or in the adjacent space, and its great dynamism with respect to the network core, which is difficult for the method to adapt.


In order to achieve highly dynamic network routing, the geographic location information of the contact forwarding nodes is mandatory to be considered.
For the node location dynamics of wireless sensor networks, geographic routing (Geographical Routing) or location-aided routing (Location-Adied Routing, LAR) Cadger \cite {cadger2012survey,mauve2001survey} based on dedicated location services \cite {li2000scalable} or GNSS systems to solve such problems, which can be divided into two major categories: Greedy Forwarding (GFR) and Face Routing (FR).
The former includes MFR\cite{takagi1984optimal}, NFP\cite{hou1986transmission}, Compass Routing\cite{kranakis1999compass}, and Random Nearest\cite{ nelson1984space}, but with no guaranteed delivery; the latter is transformed from Compass Routing II, which can guarantee delivery, but the efficiency is received due to detours \cite{kuhn2008algorithmic}.

In summary, the above methods do not sufficiently consider the characteristics of large scale, large scale, and high dynamics of space communication networks, and the proposed methods cannot simultaneously meet the requirements of distributed, low overhead, and dynamic routing at the edge of the network, which poses a challenge to the routing scheme of the future giant constellation space communication network system.


% 在空间网络中，高动态下网络的路由是决定网络实现全球长距实时通讯的是否可行的关键技术之一。而在确定路由之前，还有一些问题需要探讨，尤其是拓扑设计以及能可视化观察路由过程的仿真平台
In LEO SNs, the routing of the network under high dynamics is one of the key technologies that determine the feasibility of the network to achieve global long-range real-time communication.
In addition to this, there are several issues to be explored, especially the topology design and the simulation platform that can visualize the routing process, which is decisive for the design of the routing scheme.

% In this section, we give a brief introduction to the topology design and routing scheme of satellite networks, we also list the works that have been done on simulation platforms.


==> tab/alg.tex <==
\begin{algorithm}
    \label{alg:mplf}
    \caption{Location Forwarding of in a Single LFR}%算法名字
    \LinesNumbered %要求显示行号
    \KwIn{ last FLR $s_{in},~s_{in} \in \mathcal{V}_{adj}(s_i)$\\
        \ \ ECI Coordinations of \\
        \ \ \ \ destination LER $\mathbf{x}(s_d)$ \\
        \ \  \ \  current FLR $\mathbf{x}(s_i)$ \\
        \ \ \ \ adjacent FLRs $\mathbf{x}(s_{j}),~ s_j \in \mathcal{V}_{adj}(s_i) $
        }%输入参数
    \KwOut{outport $\mathbf{e}_{next}$}%输出

        $ \textit{cos}_{min} \leftarrow 0$\;
        $\mathbf{e}_{d}\left\langle s_i,s_d \right\rangle  =  \mathbf{x}(s_d)-\mathbf{x}(s_i)$ \;
        \For{ $s_j \in \mathcal{V}_{adj}(s_i) $  }{
            
            $\mathbf{e}(s_j) \leftarrow \mathbf{x}(s_{j}) - \mathbf{x}(s_i)$ \;

            $\textit{cos} = \mathbf{e}(s_j) \cdot \mathbf{e}_{d}\backslash ( \|\mathbf{e}(s_j)\|\|\mathbf{e}_{d}\| )$\;
            \If {$\textit{cos}_{min} \ge \textit{cos} $}{
                $\textit{cos}_{min} \leftarrow \textit{cos}$\;
                $\mathbf{e}_{next} = \mathbf{e}(s_j)$
            }
           
        }
        \If {$\textbf{e}_{last} = - \textbf{e}_{next} $}{
            drop the datagram \;
            send NACK to $\textbf{e}_{last}$
        
        }
    \end{algorithm}

==> tab/fluctuation.tex <==

\begin{table*}[t!]

    \caption{Fluctuations among cities in different routing methods.} 
    \label{tab:fluctuation}
    \centering
    \scalebox{1.3}{
    \begin{tabular}{l|cccc}
       \toprule[2pt] 
      & \multicolumn{4}{c}{\centering{Algorithms}}\\
      \cline{3-4}
      \begin{tabular}[c]{@{}c@{}}  \end{tabular}
      $LAT_{max} - LAT_{min}\backslash $ fluctuation& LH &SP&GPSR &MPLF  \\
      \hline
     \quad Harbin to London &60.12$\backslash$70.58\%&44.32$\backslash$59.45\%    &16.21$\backslash$40.33\%&30.22$\backslash$37.50\%\\
     \quad London to San Francisco&23.26$\backslash$52.87\%   &24.35$\backslash$57.14\%         &5.32$\backslash$14.88\%&35.14$\backslash$82.12\% \\
     \quad San Francisco to Shanghai &40.36$\backslash$72.72\% &30.95$\backslash$60.03\%  &n/a &15.23$\backslash$35.59\%\\
      %sildurs-10k&0.6&0.151&24&1\\
\hline
\quad Harbin to London &5.51$\backslash$17.46\%& 4.54$\backslash$14.87\%   & 7.23$\backslash$19.54\%&4.54$\backslash$14.87\%\\
\quad London to San Francisco&6.32$\backslash$17.64\%   &4.21$\backslash$6.45\%       &4.25$\backslash$11.76\%  &4.21$\backslash$6.45\% \\
\quad San Francisco to Shanghai &4.23$\backslash$12.35\% &4.23$\backslash$12.01\%  &4.23$\backslash$11.32\% &4.23$\backslash$11.32\%\\
      \toprule[2pt]
    \end{tabular}
    }
    %  \vspace{-2mm}
\end{table*}


==> tab/gses.tex <==
\begin{table*}[htbp]
	\centering
	\caption{aas}
	\label{tab:gses}
	\scalebox{1}{

		\begin{tabular}{c|cccccc}
			\toprule[2pt]

			         & GS00-GS20 & GS01-GS21 & GS02-GS22 & GS03-GS23 & GS04-GS24 & GS05-GS25 \\ \hline
			SRC      & 0E,50N    & 18E,50N   & 36E,50N   & 54E,50N   & 72E,50N   & 90E,50N   \\
			DST      & 180W,50S  & 162W,50S  & 144W,50S  & 126W,50S  & 108W,50S  & 90E,50S   \\
			Distance & 19998.15  & 17461.25  & 15062.56  & 13020.83  & 11599.87  & 11081.69  \\ 
			\toprule[2pt]

			         & GS39-GS19 & GS38-GS18 & GS37-GS17 & GS36-GS16 & GS35-GS15 &           \\ \hline
			SRC      & 0E,40N    & 0E,30N    & 0E,20N    & 0E,10N    & 0E,0N     &           \\
			DST      & 180W,40S  & 180W,30S  & 180W,20S  & 180W,10S  & 180W,0S   &           \\
			Distance & 19970.32  & 19972.31  & 19977.69  & 19984.97  & 19992.30  &           \\ 
			\toprule[2pt]
		\end{tabular}
	}
\end{table*}
